Phase Transitions on 1d Long-Range Ising Models with Decaying Fields: A Direct Proof via Contours

Following seminal work by J. Fr\"ohlich and T. Spencer on the critical exponent $\alpha=2$, we give a proof via contours of phase transition in the one-dimensional long-range ferromagnetic Ising model in the entire region of decay, where phase transition is known to occur, i.e., polynomial decay $\alpha \in (1,2]$. No assumptions that the nearest-neighbor interaction $J(1)$ is large are made. The robustness of the method also yields a proof of phase transition in the presence of a nonsummable external field that decays sufficiently fast.

==> Images/Trees.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Ellipse [id:dp08667119699707859] 
\draw   (148.29,289) .. controls (137.28,289.18) and (128.2,279.86) .. (128.01,268.2) .. controls (127.83,256.54) and (136.6,246.95) .. (147.62,246.77) .. controls (158.63,246.6) and (167.71,255.91) .. (167.89,267.57) .. controls (168.08,279.23) and (159.3,288.83) .. (148.29,289) -- cycle ;
%Shape: Ellipse [id:dp2624516351214634] 
\draw   (65.68,212.71) .. controls (54.66,212.88) and (45.59,203.57) .. (45.4,191.91) .. controls (45.22,180.25) and (53.99,170.65) .. (65,170.48) .. controls (76.02,170.3) and (85.09,179.61) .. (85.28,191.27) .. controls (85.46,202.94) and (76.69,212.53) .. (65.68,212.71) -- cycle ;
%Shape: Ellipse [id:dp18550609769324145] 
\draw   (148.16,209.94) .. controls (137.15,210.11) and (128.07,200.8) .. (127.89,189.14) .. controls (127.7,177.48) and (136.48,167.89) .. (147.49,167.71) .. controls (158.5,167.54) and (167.58,176.85) .. (167.76,188.51) .. controls (167.95,200.17) and (159.17,209.76) .. (148.16,209.94) -- cycle ;
%Straight Lines [id:da9527947529524217] 
\draw    (128.01,268.2) -- (65.68,212.71) ;
%Shape: Ellipse [id:dp15950683828633228] 
\draw   (229.32,212.03) .. controls (240.33,212.01) and (249.24,202.66) .. (249.22,191.16) .. controls (249.2,179.65) and (240.26,170.34) .. (229.25,170.37) .. controls (218.23,170.39) and (209.32,179.74) .. (209.34,191.24) .. controls (209.36,202.74) and (218.3,212.05) .. (229.32,212.03) -- cycle ;
%Straight Lines [id:da889851942525721] 
\draw    (167.97,267.87) -- (229.32,212.03) ;
%Straight Lines [id:da7955087402076708] 
\draw    (147.62,246.77) -- (148.16,209.94) ;
%Shape: Ellipse [id:dp03846345066889478] 
\draw   (65.42,133.7) .. controls (54.41,133.88) and (45.33,124.56) .. (45.15,112.9) .. controls (44.96,101.24) and (53.74,91.65) .. (64.75,91.47) .. controls (75.76,91.3) and (84.84,100.61) .. (85.02,112.27) .. controls (85.21,123.93) and (76.43,133.53) .. (65.42,133.7) -- cycle ;
%Shape: Ellipse [id:dp24575202948365593] 
\draw   (147.91,130.93) .. controls (136.89,131.11) and (127.82,121.8) .. (127.63,110.14) .. controls (127.45,98.47) and (136.22,88.88) .. (147.23,88.7) .. controls (158.25,88.53) and (167.32,97.84) .. (167.51,109.5) .. controls (167.69,121.16) and (158.92,130.76) .. (147.91,130.93) -- cycle ;
%Shape: Ellipse [id:dp11794093517144022] 
\draw   (229.06,133.02) .. controls (240.08,133) and (248.99,123.66) .. (248.97,112.15) .. controls (248.95,100.65) and (240,91.34) .. (228.99,91.36) .. controls (217.98,91.38) and (209.07,100.73) .. (209.09,112.23) .. controls (209.11,123.74) and (218.05,133.05) .. (229.06,133.02) -- cycle ;
%Straight Lines [id:da8174905377007264] 
\draw    (167.71,188.86) -- (229.06,133.02) ;
%Straight Lines [id:da9399447738363744] 
\draw    (147.36,167.77) -- (147.91,130.93) ;
%Shape: Ellipse [id:dp8308209304660052] 
\draw   (65.17,54.69) .. controls (54.15,54.87) and (45.08,45.56) .. (44.89,33.9) .. controls (44.71,22.24) and (53.48,12.64) .. (64.5,12.46) .. controls (75.51,12.29) and (84.58,21.6) .. (84.77,33.26) .. controls (84.96,44.92) and (76.18,54.52) .. (65.17,54.69) -- cycle ;
%Shape: Ellipse [id:dp3424663935584815] 
\draw   (147.65,51.93) .. controls (136.64,52.1) and (127.56,42.79) .. (127.38,31.13) .. controls (127.19,19.47) and (135.97,9.87) .. (146.98,9.7) .. controls (157.99,9.52) and (167.07,18.83) .. (167.25,30.5) .. controls (167.44,42.16) and (158.66,51.75) .. (147.65,51.93) -- cycle ;
%Straight Lines [id:da30583498501843986] 
\draw    (127.5,110.19) -- (65.17,54.69) ;
%Shape: Ellipse [id:dp3547548368549749] 
\draw   (228.81,54.02) .. controls (239.82,53.99) and (248.73,44.65) .. (248.71,33.14) .. controls (248.69,21.64) and (239.75,12.33) .. (228.74,12.36) .. controls (217.72,12.38) and (208.81,21.72) .. (208.83,33.23) .. controls (208.85,44.73) and (217.8,54.04) .. (228.81,54.02) -- cycle ;
%Straight Lines [id:da8325642057332256] 
\draw    (167.46,109.86) -- (228.81,54.02) ;
%Straight Lines [id:da781745467254753] 
\draw    (147.11,88.76) -- (147.65,51.93) ;
%Straight Lines [id:da8990513216000928] 
\draw    (65,170.48) -- (65.55,133.65) ;
%Right Arrow [id:dp6103345234733022] 
%\draw   (291,136) -- (333,136) -- (333,126) -- (361,146) -- (333,166) -- (333,156) -- (291,156) -- cycle ;
%Shape: Ellipse [id:dp027750399010713966] 
\draw   (508.29,285.68) .. controls (497.28,285.86) and (488.2,276.55) .. (488.01,264.89) .. controls (487.83,253.22) and (496.6,243.63) .. (507.62,243.45) .. controls (518.63,243.28) and (527.71,252.59) .. (527.89,264.25) .. controls (528.08,275.91) and (519.3,285.51) .. (508.29,285.68) -- cycle ;
%Shape: Ellipse [id:dp6479653521325581] 
\draw   (425.68,209.39) .. controls (414.66,209.56) and (405.59,200.25) .. (405.4,188.59) .. controls (405.22,176.93) and (413.99,167.33) .. (425,167.16) .. controls (436.02,166.98) and (445.09,176.3) .. (445.28,187.96) .. controls (445.46,199.62) and (436.69,209.21) .. (425.68,209.39) -- cycle ;
%Shape: Ellipse [id:dp8102407993115321] 
\draw   (508.16,206.62) .. controls (497.15,206.8) and (488.07,197.49) .. (487.89,185.82) .. controls (487.7,174.16) and (496.48,164.57) .. (507.49,164.39) .. controls (518.5,164.22) and (527.58,173.53) .. (527.76,185.19) .. controls (527.95,196.85) and (519.17,206.45) .. (508.16,206.62) -- cycle ;
%Straight Lines [id:da7252106457848171] 
\draw    (488.01,264.89) -- (425.68,209.39) ;
%Shape: Ellipse [id:dp38472605715244956] 
\draw   (589.32,208.71) .. controls (600.33,208.69) and (609.24,199.34) .. (609.22,187.84) .. controls (609.2,176.34) and (600.26,167.03) .. (589.25,167.05) .. controls (578.23,167.07) and (569.32,176.42) .. (569.34,187.92) .. controls (569.36,199.43) and (578.3,208.74) .. (589.32,208.71) -- cycle ;
%Straight Lines [id:da4181629050705957] 
\draw    (527.97,264.55) -- (589.32,208.71) ;
%Straight Lines [id:da6701149507379303] 
\draw    (507.62,243.45) -- (508.16,206.62) ;
%Shape: Ellipse [id:dp5972109252519358] 
\draw   (425.42,130.38) .. controls (414.41,130.56) and (405.33,121.25) .. (405.15,109.59) .. controls (404.96,97.92) and (413.74,88.33) .. (424.75,88.15) .. controls (435.76,87.98) and (444.84,97.29) .. (445.02,108.95) .. controls (445.21,120.61) and (436.43,130.21) .. (425.42,130.38) -- cycle ;
%Shape: Ellipse [id:dp6438666096548735] 
\draw   (507.91,127.62) .. controls (496.89,127.79) and (487.82,118.48) .. (487.63,106.82) .. controls (487.45,95.16) and (496.22,85.56) .. (507.23,85.39) .. controls (518.25,85.21) and (527.32,94.52) .. (527.51,106.19) .. controls (527.69,117.85) and (518.92,127.44) .. (507.91,127.62) -- cycle ;
%Shape: Ellipse [id:dp6010157642496443] 
\draw   (589.06,129.71) .. controls (600.08,129.68) and (608.99,120.34) .. (608.97,108.83) .. controls (608.95,97.33) and (600,88.02) .. (588.99,88.04) .. controls (577.98,88.07) and (569.07,97.41) .. (569.09,108.92) .. controls (569.11,120.42) and (578.05,129.73) .. (589.06,129.71) -- cycle ;
%Straight Lines [id:da8863179534346235] 
\draw    (527.71,185.55) -- (589.06,129.71) ;
%Straight Lines [id:da6690391080911193] 
\draw    (507.36,164.45) -- (507.91,127.62) ;
%Straight Lines [id:da5152694348201234] 
\draw    (425,167.16) -- (425.55,130.33) ;

% Text Node
\draw (310,130.4) node [anchor=north west][inner sep=0.75pt]    { \huge $\Rightarrow$};

% Text Node
\draw (250,260.4) node [anchor=north west][inner sep=0.75pt]    {\Large $T$};
% Text Node
\draw (144,258.4) node [anchor=north west][inner sep=0.75pt]    {$0$};
% Text Node
\draw (47,183.4) node [anchor=north west][inner sep=0.75pt]    {$(1,1)$};
% Text Node
\draw (129,180) node [anchor=north west][inner sep=0.75pt]    {$(1,2)$};
% Text Node
\draw (210,183) node [anchor=north west][inner sep=0.75pt]    {$(1,3)$};
% Text Node
\draw (47,103.4) node [anchor=north west][inner sep=0.75pt]    {$(2,1)$};
% Text Node
\draw (130,102.4) node [anchor=north west][inner sep=0.75pt]    {$(2,2)$};
% Text Node
\draw (212,104.4) node [anchor=north west][inner sep=0.75pt]    {$(2,3)$};
% Text Node
\draw (45,25.4) node [anchor=north west][inner sep=0.75pt]    {$(3,1)$};
% Text Node
\draw (129,20) node [anchor=north west][inner sep=0.75pt]    {$(3,2)$};
% Text Node
\draw (209,24.4) node [anchor=north west][inner sep=0.75pt]    {$(3,3)$};
% Text Node
\draw (610,257.08) node [anchor=north west][inner sep=0.75pt]    {\Large $T_1$};
% Text Node
\draw (504,255.08) node [anchor=north west][inner sep=0.75pt]    {$0$};
% Text Node
\draw (407,180.08) node [anchor=north west][inner sep=0.75pt]    {$(1,1)$};
% Text Node
\draw (489,179.08) node [anchor=north west][inner sep=0.75pt]    {$(1,2)$};
% Text Node
\draw (571,179.08) node [anchor=north west][inner sep=0.75pt]    {$(1,3)$};
% Text Node
\draw (407,100.08) node [anchor=north west][inner sep=0.75pt]    {$(2,1)$};
% Text Node
\draw (490,99.08) node [anchor=north west][inner sep=0.75pt]    {$(2,2)$};
% Text Node
\draw (572,101.08) node [anchor=north west][inner sep=0.75pt]    {$(2,3)$};


\end{tikzpicture}

==> Images/Trees2.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,409); %set diagram left start at 0, and has height of 409

%Shape: Circle [id:dp9870314440900954] 
\draw   (291,345) .. controls (291,331.19) and (302.19,320) .. (316,320) .. controls (329.81,320) and (341,331.19) .. (341,345) .. controls (341,358.81) and (329.81,370) .. (316,370) .. controls (302.19,370) and (291,358.81) .. (291,345) -- cycle ;
%Shape: Circle [id:dp6884461835409985] 
\draw   (138,247) .. controls (138,233.19) and (149.19,222) .. (163,222) .. controls (176.81,222) and (188,233.19) .. (188,247) .. controls (188,260.81) and (176.81,272) .. (163,272) .. controls (149.19,272) and (138,260.81) .. (138,247) -- cycle ;
%Shape: Circle [id:dp22929770844962816] 
\draw   (292,219) .. controls (292,205.19) and (303.19,194) .. (317,194) .. controls (330.81,194) and (342,205.19) .. (342,219) .. controls (342,232.81) and (330.81,244) .. (317,244) .. controls (303.19,244) and (292,232.81) .. (292,219) -- cycle ;
%Shape: Circle [id:dp8997196501569942] 
\draw   (437,241) .. controls (437,227.19) and (448.19,216) .. (462,216) .. controls (475.81,216) and (487,227.19) .. (487,241) .. controls (487,254.81) and (475.81,266) .. (462,266) .. controls (448.19,266) and (437,254.81) .. (437,241) -- cycle ;
%Shape: Circle [id:dp8873903066291231] 
\draw   (55,137) .. controls (55,123.19) and (66.19,112) .. (80,112) .. controls (93.81,112) and (105,123.19) .. (105,137) .. controls (105,150.81) and (93.81,162) .. (80,162) .. controls (66.19,162) and (55,150.81) .. (55,137) -- cycle ;
%Shape: Circle [id:dp2808811450363127] 
\draw   (141,118) .. controls (141,104.19) and (152.19,93) .. (166,93) .. controls (179.81,93) and (191,104.19) .. (191,118) .. controls (191,131.81) and (179.81,143) .. (166,143) .. controls (152.19,143) and (141,131.81) .. (141,118) -- cycle ;
%Shape: Circle [id:dp10143913655723802] 
\draw   (228,114) .. controls (228,100.19) and (239.19,89) .. (253,89) .. controls (266.81,89) and (278,100.19) .. (278,114) .. controls (278,127.81) and (266.81,139) .. (253,139) .. controls (239.19,139) and (228,127.81) .. (228,114) -- cycle ;
%Shape: Circle [id:dp14916133075598337] 
\draw   (303,103) .. controls (303,89.19) and (314.19,78) .. (328,78) .. controls (341.81,78) and (353,89.19) .. (353,103) .. controls (353,116.81) and (341.81,128) .. (328,128) .. controls (314.19,128) and (303,116.81) .. (303,103) -- cycle ;
%Shape: Circle [id:dp07990395389801086] 
\draw   (380,113) .. controls (380,99.19) and (391.19,88) .. (405,88) .. controls (418.81,88) and (430,99.19) .. (430,113) .. controls (430,126.81) and (418.81,138) .. (405,138) .. controls (391.19,138) and (380,126.81) .. (380,113) -- cycle ;
%Shape: Circle [id:dp44859639892607595] 
\draw   (484,126) .. controls (484,112.19) and (495.19,101) .. (509,101) .. controls (522.81,101) and (534,112.19) .. (534,126) .. controls (534,139.81) and (522.81,151) .. (509,151) .. controls (495.19,151) and (484,139.81) .. (484,126) -- cycle ;
%Straight Lines [id:da34927395168393716] 
\draw    (179,266) -- (291,342) ;
%Straight Lines [id:da2153422225050292] 
\draw    (316,244) -- (316,320) ;
%Straight Lines [id:da40468327569148643] 
\draw    (341,345) -- (447,260.8) ;
%Straight Lines [id:da3425912636611841] 
\draw    (89.2,160.4) -- (145.4,229.6) ;
%Straight Lines [id:da9336347983580622] 
\draw    (166,143) -- (167,221.8) ;
%Straight Lines [id:da7257339071297162] 
\draw    (253,139) -- (300,200) ;
%Straight Lines [id:da6441165631203483] 
\draw    (328,128) -- (319.6,194.4) ;
%Straight Lines [id:da2825912381547342] 
\draw    (394.4,136) -- (337.8,203.4) ;
%Straight Lines [id:da9800601415687946] 
\draw    (468.6,216.6) -- (501.8,150.2) ;
%Shape: Rectangle [id:dp3630669612916777] 
\draw   (40.58,93.45) -- (189.23,67.91) -- (205,159.67) -- (56.35,185.21) -- cycle ;
%Shape: Rectangle [id:dp17656067327416003] 
\draw   (222.21,59.72) -- (443.65,69.7) -- (439.46,162.61) -- (218.02,152.63) -- cycle ;
%Shape: Rectangle [id:dp6608700789820505] 
\draw   (474,81.28) -- (558.01,94.23) -- (547,165.72) -- (462.99,152.77) -- cycle ;

% Text Node
\draw (309.33,332.73) node [anchor=north west][inner sep=0.75pt]  [font=\Large]  {$0$};
% Text Node
\draw (141.67,236.73) node [anchor=north west][inner sep=0.75pt]    {$( 1,\ 1)$};
% Text Node
\draw (296,208.4) node [anchor=north west][inner sep=0.75pt]    {$( 1,\ 2)$};
% Text Node
\draw (441.33,231.4) node [anchor=north west][inner sep=0.75pt]    {$( 1,\ 3)$};
% Text Node
\draw (59,126.4) node [anchor=north west][inner sep=0.75pt]    {$( 2,\ 1)$};
% Text Node
\draw (144.67,107.07) node [anchor=north west][inner sep=0.75pt]    {$( 2,\ 2)$};
% Text Node
\draw (232,104.4) node [anchor=north west][inner sep=0.75pt]    {$( 2,\ 3)$};
% Text Node
\draw (306.67,93.73) node [anchor=north west][inner sep=0.75pt]    {$( 2,\ 4)$};
% Text Node
\draw (383.33,102.73) node [anchor=north west][inner sep=0.75pt]    {$( 2,\ 5)$};
% Text Node
\draw (488.67,114.4) node [anchor=north west][inner sep=0.75pt]    {$( 2,\ 6)$};
% Text Node
\draw (75.22,54.21) node [anchor=north west][inner sep=0.75pt]  [font=\large,rotate=-352.63]  {$q\ =\ 1$};
% Text Node
\draw (310.26,35.97) node [anchor=north west][inner sep=0.75pt]  [font=\large,rotate=-1.52]  {$q\ =\ 2$};
% Text Node
\draw (500.77,57.17) node [anchor=north west][inner sep=0.75pt]  [font=\large,rotate=-8.76]  {$q\ =\ 3$};


\end{tikzpicture}
